DCFormer: Efficient 3D Vision-Language Modeling with Decomposed Convolutions

Vision-language models (VLMs) have been widely applied to 2D medical image analysis due to their ability to align visual and textual representations. However, extending VLMs to 3D imaging remains computationally challenging. Existing 3D VLMs often rely on Vision Transformers (ViTs), which are computationally expensive due to the quadratic complexity of self-attention, or on 3D convolutions, which require large numbers of parameters and FLOPs as kernel size increases. We introduce DCFormer, an efficient 3D image encoder that factorizes 3D convolutions into three parallel 1D convolutions along the depth, height, and width dimensions. This design preserves spatial information while significantly reducing computational cost. Integrated into a CLIP-based vision-language framework, DCFormer is trained and evaluated on CT-RATE, a dataset of 50,188 paired 3D chest CT volumes and radiology reports. In zero-shot and fine-tuned detection of 18 pathologies, as well as in image-text retrieval tasks, DCFormer consistently outperforms state-of-the-art 3D vision encoders, including CT-ViT, ViT, ConvNeXt, PoolFormer, and TransUNet. These results highlight DCFormer's potential for scalable, clinically deployable 3D medical VLMs. Our code is available at: https://github.com/mirthAI/DCFormer.

==> figures/conv_flop.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=10cm]{figures/conv_flop.png}\\
\caption{\textcolor{red}{FLOP and parameter comparison of 2D and 3D convolutions. For simplicity, we set the number of output channels $C=32$ and depth dimension $D=32$}}
\label{fig:convflop} 
\end{figure*}


==> figures/flop.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=10cm]{figures/flop.png}\\
\caption{FLOP and parameter comparison between depthwise convolution and decomposed depthwise convolution.}
\label{fig:flop} 
\end{figure*}


==> tables/config_copy.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\caption{\label{config} Architectural configurations of the DCFormer model variants.}
\begin{tabular}{|llll|cccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Stage}} & \multicolumn{1}{c|}{\multirow{2}{*}{\#Tokens}}            & \multicolumn{2}{c|}{\multirow{2}{*}{Layer Specification}}                             & \multicolumn{4}{c|}{DCFormer}                                                            \\ \cline{5-8} 
\multicolumn{1}{|c|}{}                       & \multicolumn{1}{c|}{}                                    & \multicolumn{2}{l|}{}                                                                 & \multicolumn{1}{c|}{Nano}     & \multicolumn{1}{c|}{Naive}     & \multicolumn{1}{c|}{Tiny}     & Small     \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{0}}     & \multicolumn{1}{l|}{\multirow{4}{*}{H/4 X W/4 X D/4}}    & \multicolumn{1}{l|}{\multirow{4}{*}{STEM}}               & Embed. Dim.                & \multicolumn{2}{c|}{32}       & \multicolumn{2}{c|}{64}              \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & \#Blocks                    & \multicolumn{4}{c|}{4}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Patch size (block 1)       & \multicolumn{4}{c|}{7 x 7 x 7, stride 4}                                                     \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Patch size (block 2, 3, 4) & \multicolumn{4}{c|}{3 x 3 x 3, stride 1}                                                     \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{1}}     & \multicolumn{1}{l|}{\multirow{5}{*}{H/8 X W/8 X D/8}}    & \multicolumn{1}{l|}{\multirow{2}{*}{Patch Embedding}}    & Patch size                 & \multicolumn{4}{c|}{3 x 3 x 3, stride 2}                                                     \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Embed. Dim.                & \multicolumn{1}{c|}{32}    & \multicolumn{1}{c|}{64}    & \multicolumn{2}{c|}{96}            \\ \cline{3-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{\multirow{3}{*}{DCFormer Block}} & Kernel size                & \multicolumn{4}{c|}{7}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & MLP Ratio                  & \multicolumn{4}{c|}{4}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & \#Blocks                    & \multicolumn{1}{c|}{1}     & \multicolumn{3}{c|}{2}                                          \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{2}}     & \multicolumn{1}{l|}{\multirow{5}{*}{H/16 X W/16 X D/16}} & \multicolumn{1}{l|}{\multirow{2}{*}{Patch Embedding}}    & Patch size                 & \multicolumn{4}{c|}{3 x 3 x 3, stride 2}                                                     \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Embed. Dim.                & \multicolumn{1}{c|}{64}    & \multicolumn{1}{c|}{128}   & \multicolumn{2}{c|}{192}           \\ \cline{3-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{\multirow{3}{*}{DCFormer Block}} & Kernel size                & \multicolumn{4}{c|}{7}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & MLP Ratio                  & \multicolumn{4}{c|}{4}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & \#Blocks                    & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{2}     & \multicolumn{2}{c|}{3}             \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{3}}     & \multicolumn{1}{l|}{\multirow{5}{*}{H/32 X W/32 X D/32}} & \multicolumn{1}{l|}{\multirow{2}{*}{Patch Embedding}}    & Patch size                 & \multicolumn{4}{c|}{3 x 3 x 3, stride 2}                                                     \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Embed. Dim.                & \multicolumn{1}{c|}{128}   & \multicolumn{1}{c|}{256}   & \multicolumn{2}{c|}{384}           \\ \cline{3-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{\multirow{3}{*}{DCFormer Block}} & Kernel size                & \multicolumn{4}{c|}{7}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & MLP Ratio                  & \multicolumn{4}{c|}{4}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & \#Blocks                    & \multicolumn{1}{c|}{1}     & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{3}     & 6     \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{4}}     & \multicolumn{1}{l|}{\multirow{5}{*}{H/64 X W/64 X D/64}} & \multicolumn{1}{l|}{\multirow{2}{*}{Patch Embedding}}    & Patch size                 & \multicolumn{4}{c|}{3 x 3 x 3, stride 2}                                                     \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & Embed. Dim.                & \multicolumn{1}{c|}{256}   & \multicolumn{1}{c|}{512}   & \multicolumn{2}{c|}{768}           \\ \cline{3-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{\multirow{3}{*}{DCFormer Block}} & Kernel size                & \multicolumn{4}{c|}{7}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & MLP Ratio                  & \multicolumn{4}{c|}{4}                                                                       \\ \cline{4-8} 
\multicolumn{1}{|l|}{}                       & \multicolumn{1}{l|}{}                                    & \multicolumn{1}{l|}{}                                    & \#Blocks                    & \multicolumn{1}{c|}{1}     & \multicolumn{3}{c|}{2}                                          \\ \hline
\multicolumn{4}{|c|}{Parameters (M)}                                                                                                                                                            & \multicolumn{1}{c|}{0.92} & \multicolumn{1}{c|}{5.85} & \multicolumn{1}{c|}{15.1} & 26.86 \\ \hline
\multicolumn{4}{|c|}{FLOPS(G)}                                                                                                                                                                  & \multicolumn{1}{c|}{34.21} & \multicolumn{1}{c|}{49.48} & \multicolumn{1}{c|}{168.2} & 202.9 \\ \hline
\end{tabular}
\end{center}

\end{table*}

==> tables/paramflop.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Layer}        & \textbf{2D Convolution}                            & \textbf{3D Convolution}                              & \textbf{2D Depthwise Convolution}                   & \textbf{3D Depthwise Convolution}                   \\ \hline
\textbf{Parameters}     & $k_h \cdot k_w \cdot C_{\text{in}} \cdot C_{\text{out}}$ & $k_d \cdot k_h \cdot k_w \cdot C_{\text{in}} \cdot C_{\text{out}}$ & $k_h \cdot k_w \cdot C_{\text{in}}$    & $k_d \cdot k_h \cdot k_w \cdot C_{\text{in}}$    \\ \hline
\textbf{FLOPs}          & $ 2 \cdot H \cdot W \cdot C_{\text{out}} \cdot C_{\text{in}} \cdot k_h \cdot k_w$ & $2 \cdot D \cdot H \cdot W \cdot C_{\text{out}} \cdot C_{\text{in}} \cdot k_d \cdot k_h \cdot k_w$ & $2 \cdot H \cdot W \cdot C_{\text{in}} \cdot k_h \cdot k_w$ & $2 \cdot D \cdot H \cdot W \cdot C_{\text{in}} \cdot k_d \cdot k_h \cdot k_w$ \\ \hline
\textbf{Scaling Factor (Params)}  & $C_{\text{out}}$  & $k_d \cdot C_{\text{out}}$              & 1                                         & $k_d $      \\ \hline
\textbf{Scaling Factor (FLOPs)}   & $C_{\text{out}}$                 & $k_d \cdot D \cdot C_{\text{out}}$              & $1$                  & $k_d \cdot D$      \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of parameters and FLOPs for 2D and 3D convolutions, including depthwise convolutions. Here, \(k_h\), \(k_w\), and \(k_d\) represent the height, width, and depth of the convolution kernel, respectively. \(C_{\text{in}}\) denotes the number of input channels, and \(C_{\text{out}}\) represents the number of output channels. \(H\), \(W\), and \(D\) correspond to the height, width, and depth of the feature map, respectively.}
\label{tab:conv_comparison}
\end{table*}


==> tables/results.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{model} & \textbf{variant} & \textbf{params (M)} & \textbf{GFLOPS} & \textbf{accuracy (\%)} & \textbf{f1 score (\%)} & \textbf{precision (\%)} & \textbf{recall (\%)} \\ \hline
        \textbf{DCFormer} & nano & 920.3K & 34.21 & 60.4 & 41.9 & 27.2 & 62.8 \\ \hline
        %\textbf{inceptionnext} & nano & ~ & ~ & 1.80M & 19.77G & ~ & ~ \\ \hline
        \textbf{convnext \cite{liu2022convnet}} & nano & 3.19M & 31.92 & 62.2 & 39.4 & 26.7 & 55.1 \\ \hline
        \textbf{poolformer \cite{yu2022metaformer}} & nano & 2.79M & 27.14 & 60.2 & 37.0 & 24.8 & 52.3 \\ \hline
        %\textbf{DCFormer} & naïve & 13-11-9-7 & C-C-C-C & 6.20M & 139.3G & 65.6 & 45.6 \\ \hline
        \textbf{DCFormer} & naïve & 5.85M & 49.48 & 63.1 & 44.5 & 29.5 & 65.5 \\ \hline
        \textbf{vit \cite{dosovitskiy2020image}} & naïve & 11.10M & 39.05 & 55 & 42.5 & 25.8 & 71.5 \\ \hline
        %\textbf{inceptionnext} & naïve & ~ & ~ & 9.24M & 60.10G & ~ & ~ \\ \hline  
        \textbf{convnext \cite{liu2022convnet}} & naive & 15.63M & 96.84 & 60.7 & 42.4 & 27.7 & 63.8 \\ \hline        
        \textbf{poolformer \cite{yu2022metaformer}} & naïve & 11.31M & 63.75 & 60.1 & 39.1 & 25.7 & 56.8 \\ \hline
        \textbf{transunet \cite{chen2021transunet}} & naïve & 12.48M & 118.9 & 58.6 & 41.4 & 26.5 & 56.0 \\ \hline
        \textbf{DCFormer} & tiny & 15.1M & 168.2 & 62.0 & 46.3 & 29.7 & 70.1 \\ \hline
        \textbf{vit \cite{dosovitskiy2020image}} & tiny & 26.34M & 86.43 & 61 & 43.2 & 28.0 & 64.8 \\ \hline
        \textbf{convnext \cite{liu2022convnet}} & tiny & 31.59M & 156.31 & 62.5 & 42.1 & 28.2 & 60.1 \\ \hline
        %\textbf{inceptionnext} & tiny & ~ & ~ & 29.39M & 140.9G & ~ & ~ \\ \hline
        \textbf{transunet \cite{chen2021transunet}} & tiny & 23.93M & 207.5 & 61.5 & 35.8 & 24.7 & 48.7 \\ \hline
        \textbf{poolformer \cite{yu2022metaformer}} & tiny & 20.68M & 117.46 & 61.8 & 38.3 & 26.0 & 53.5 \\ \hline        
        %\textbf{DCFormer} & small & 7-7-7-7 & C-C-T-T & 26.86M & 202.9G & ~ & ~ \\ \hline
        %\textbf{vit} & small & ~ & ~ & 45.81M & 142.5G & 62.8 & 44.5 \\ \hline
        %\textbf{transunet} & small & ~ & ~ & 62.46M & 467.8G & ~ & ~ \\ \hline
        %\textbf{convnext} & small & ~ & ~ & 55.26M & 207.7G & ~ & ~ \\ \hline
        %\textbf{inceptionnext} & small & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        %\textbf{poolformer} & small & ~ & ~ & 50.64M & 184.1G & ~ & ~ \\ \hline
        \textbf{ctvit \cite{hamamci2024foundation}} & - & 101.1M & 160.5 & 62.9 & 44.3 & 29.3 & 65.7 \\ \hline
    \end{tabular}
\end{center}
\caption{\label{results} Zero-shot performance of models trained on CT-RATE dataset at the resolution of 512x512x256.}
\end{table*}



==> tables/results2.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{model} & \textbf{variant} & \textbf{kernel} & \textbf{strategy} & \textbf{params} & \textbf{flops} & \textbf{acc} & \textbf{f1} \\ \hline
        \textbf{decomp} & nano & 7-7-7-7 & C-C-C-C & 918.2K & 34.12G & ~ & ~ \\ \hline
        \textbf{decomp} & nano & 13-11-9-7 & C-C-C-C & 920.3K & 34.21G & ~ & ~ \\ \hline
        \textbf{decomp} & nano & 7-7-7-7 & C-C-T-T & 1.24M & 35.42G & ~ & ~ \\ \hline
        \textbf{inceptionnext} & nano & ~ & ~ & 1.80M & 19.77G & ~ & ~ \\ \hline
        \textbf{convnext} & nano & ~ & ~ & 3.19M & 31.92G & ~ & ~ \\ \hline
        \textbf{poolformer} & nano & ~ & ~ & 2.79M & 27.14G & ~ & ~ \\ \hline
        \textbf{decomp} & naïve & 7-7-7-7 & C-C-C-C & 6.19M & 139.1G & ~ & ~ \\ \hline
        \textbf{decomp} & naïve & 13-11-9-7 & C-C-C-C & 6.20M & 139.3G & ~ & ~ \\ \hline
        \textbf{decomp} & naïve & 7-7-7-7 & C-C-T-T & 8.81M & 145.1G & 66.2 & 45.2 \\ \hline
        \textbf{vit} & naïve & ~ & ~ & 11.10M & 39.05G & 55 & 42.5 \\ \hline
        \textbf{inceptionnext} & naïve & ~ & ~ & 9.24M & 60.10G & ~ & ~ \\ \hline        
        \textbf{poolformer} & naïve & ~ & ~ & 11.31M & 63.75G & ~ & ~ \\ \hline
        \textbf{transunet} & naïve & ~ & ~ & 12.48M & 118.9G & ~ & ~ \\ \hline
        \textbf{decomp} & tiny & 7-7-7-7 & C-C-C-C & 15.03M & 167.6G & ~ & ~ \\ \hline
        \textbf{decomp} & tiny & 13-11-9-7 & C-C-C-C & 15.1M & 168.2G & ~ & ~ \\ \hline
        \textbf{decomp} & tiny & 7-7-7-7 & C-C-T-T & 21.51M & 182.2G & ~ & ~ \\ \hline
        \textbf{vit} & tiny & ~ & ~ & 26.34M & 86.43G & 61 & 43.2 \\ \hline
        \textbf{convnext} & tiny & ~ & ~ & 31.59M & 156.31G & ~ & ~ \\ \hline
        \textbf{inceptionnext} & tiny & ~ & ~ & 29.39M & 140.9G & ~ & ~ \\ \hline
        \textbf{transunet} & tiny & ~ & ~ & 23.93M & 207.5G & ~ & ~ \\ \hline
        \textbf{poolformer} & tiny & ~ & ~ & 20.68M & 117.46G & ~ & ~ \\ \hline        
        \textbf{decomp} & small & 7-7-7-7 & C-C-T-T & 26.86M & 202.9G & ~ & ~ \\ \hline
        \textbf{vit} & small & ~ & ~ & 45.81M & 142.5G & 62.8 & 44.5 \\ \hline
        \textbf{transunet} & small & ~ & ~ & 62.46M & 467.8G & ~ & ~ \\ \hline
        \textbf{convnext} & small & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        \textbf{inceptionnext} & small & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        \textbf{poolformer} & small & ~ & ~ & 50.64M & 184.1G & ~ & ~ \\ \hline
        \textbf{ctvit} & ~ & ~ & ~ & 101.1M & 160.5G & 63 & 44.2 \\ \hline
    \end{tabular}
\end{center}
\caption{\label{results} Zero-shot performance of models trained on CT-RATE dataset at the resolution of 512x512x256.}
\end{table*}


==> tables/results_finetune.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{model} & \textbf{variant} & \textbf{params (M)} & \textbf{GFLOPS} & \textbf{accuracy (\%)} & \textbf{f1 score (\%)} & \textbf{precision (\%)} & \textbf{recall (\%)} \\ \hline
        \textbf{DCFormer} & nano & 920.3K & 34.21 & 60.1 & 45.0 & 28.6 & 69.6 \\ \hline
        %\textbf{inceptionnext} & nano & ~ & ~ & 1.80M & 19.77G & ~ & ~ \\ \hline
        \textbf{convnext \cite{liu2022convnet}} & nano & 3.19M & 31.92 & 56.3 & 43.5 & 26.2 & 70.1 \\ \hline
        \textbf{poolformer \cite{yu2022metaformer}} & nano & 2.79M & 27.14 & 52.6 & 41.2 & 24.1 & 67.6 \\ \hline
        %\textbf{DCFormer} & naïve & 13-11-9-7 & C-C-C-C & 6.20M & 139.3G & 65.6 & 45.6 \\ \hline
        \textbf{DCFormer} & naïve & 5.85M & 49.48 & 64.2 & 47.2 & 31.0 & 70.2 \\ \hline
        \textbf{vit \cite{dosovitskiy2020image}} & naïve & 11.10M & 39.05 & 56.2 & 43.1 & 26.1 & 69.8 \\ \hline
        %\textbf{inceptionnext} & naïve & ~ & ~ & 9.24M & 60.10G & ~ & ~ \\ \hline  
        \textbf{convnext \cite{liu2022convnet}} & naive & 15.63M & 96.84 & 59.0 & 44.2 & 27.2 & 67.6 \\ \hline        
        \textbf{poolformer \cite{yu2022metaformer}} & naïve & 11.31M & 63.75 & 53.9 & 41.9 & 24.8 & 68.7 \\ \hline
        \textbf{transunet \cite{chen2021transunet}} & naïve & 12.48M & 118.9 & 60.2 & 44.6 & 29.4 & 70.1 \\ \hline
        \textbf{DCFormer} & tiny & 15.1M & 168.2 & 64.1 & 48.6 & 31.4 & 72.9 \\ \hline
        \textbf{vit \cite{dosovitskiy2020image}} & tiny & 26.34M & 86.43 & 59.4 & 44.9 & 28.0 & 70.8 \\ \hline
        \textbf{convnext \cite{liu2022convnet}} & tiny & 31.59M & 156.31 & 60.4 & 44.8 & 28.2 & 68.2 \\ \hline
        %\textbf{inceptionnext} & tiny & ~ & ~ & 29.39M & 140.9G & ~ & ~ \\ \hline
        \textbf{transunet \cite{chen2021transunet}} & tiny & 23.93M & 207.5 & 50.2 & 39.4 & 22.7 & 66.1 \\ \hline
        \textbf{poolformer \cite{yu2022metaformer}} & tiny & 20.68M & 117.46 & 54.2 & 42.2 & 25.0 & 68.8 \\ \hline        
        %\textbf{DCFormer} & small & 7-7-7-7 & C-C-T-T & 26.86M & 202.9G & ~ & ~ \\ \hline
        %\textbf{vit} & small & ~ & ~ & 45.81M & 142.5G & 62.8 & 44.5 \\ \hline
        %\textbf{transunet} & small & ~ & ~ & 62.46M & 467.8G & ~ & ~ \\ \hline
        %\textbf{convnext} & small & ~ & ~ & 55.26M & 207.7G & ~ & ~ \\ \hline
        %\textbf{inceptionnext} & small & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        %\textbf{poolformer} & small & ~ & ~ & 50.64M & 184.1G & ~ & ~ \\ \hline
        \textbf{ctvit \cite{hamamci2024foundation}} & - & 101.1M & 160.5 & 61.8 & 46.4 & 29.4 & 70.1 \\ \hline
    \end{tabular}
\end{center}
\caption{\label{results_finetune} Fine-tuning performance of models trained on CT-RATE dataset at the resolution of 512x512x256.}
\end{table*}


==> tables/results_noref.tex <==
\begin{table*}[t]
\scriptsize
\renewcommand\arraystretch{1.4}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{model} & \textbf{variant} & \textbf{params (M)} & \textbf{GFLOPS} & \textbf{accuracy (\%)} & \textbf{f1 score (\%)} & \textbf{precision (\%)} & \textbf{recall (\%)} \\ \hline
        \textbf{DCFormer} & nano & 920.3K & 34.21 & 60.4 & 41.9 & 27.2 & 62.8 \\ \hline
        %\textbf{inceptionnext} & nano & ~ & ~ & 1.80M & 19.77G & ~ & ~ \\ \hline
        \textbf{convnext} & nano & 3.19M & 31.92 & 62.2 & 39.4 & 26.7 & 55.1 \\ \hline
        \textbf{poolformer} & nano & 2.79M & 27.14 & 60.2 & 37.0 & 24.8 & 52.3 \\ \hline
        %\textbf{DCFormer} & naïve & 13-11-9-7 & C-C-C-C & 6.20M & 139.3G & 65.6 & 45.6 \\ \hline
        \textbf{DCFormer} & naïve & 5.85M & 49.48 & 63.1 & 44.5 & 29.5 & 65.5 \\ \hline
        \textbf{vit} & naïve & 11.10M & 39.05 & 55 & 42.5 & 25.8 & 71.5 \\ \hline
        %\textbf{inceptionnext} & naïve & ~ & ~ & 9.24M & 60.10G & ~ & ~ \\ \hline  
        \textbf{convnext} & naive & 15.63M & 96.84 & 60.7 & 42.4 & 27.7 & 63.8 \\ \hline        
        \textbf{poolformer} & naïve & 11.31M & 63.75 & 60.1 & 39.1 & 25.7 & 56.8 \\ \hline
        \textbf{transunet} & naïve & 12.48M & 118.9 & 58.6 & 41.4 & 26.5 & 56.0 \\ \hline
        \textbf{DCFormer} & tiny & 15.1M & 168.2 & 62.0 & 46.3 & 29.7 & 70.1 \\ \hline
        \textbf{vit} & tiny & 26.34M & 86.43 & 61 & 43.2 & 28.0 & 64.8 \\ \hline
        \textbf{convnext} & tiny & 31.59M & 156.31 & 62.5 & 42.1 & 28.2 & 60.1 \\ \hline
        %\textbf{inceptionnext} & tiny & ~ & ~ & 29.39M & 140.9G & ~ & ~ \\ \hline
        \textbf{transunet} & tiny & 23.93M & 207.5 & 61.5 & 35.8 & 24.7 & 48.7 \\ \hline
        \textbf{poolformer} & tiny & 20.68M & 117.46 & 61.8 & 38.3 & 26.0 & 53.5 \\ \hline        
        %\textbf{DCFormer} & small & 7-7-7-7 & C-C-T-T & 26.86M & 202.9G & ~ & ~ \\ \hline
        %\textbf{vit} & small & ~ & ~ & 45.81M & 142.5G & 62.8 & 44.5 \\ \hline
        %\textbf{transunet} & small & ~ & ~ & 62.46M & 467.8G & ~ & ~ \\ \hline
        %\textbf{convnext} & small & ~ & ~ & 55.26M & 207.7G & ~ & ~ \\ \hline
        %\textbf{inceptionnext} & small & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
        %\textbf{poolformer} & small & ~ & ~ & 50.64M & 184.1G & ~ & ~ \\ \hline
        \textbf{ctvit} & - & 101.1M & 160.5 & 62.9 & 44.3 & 29.3 & 65.7 \\ \hline
    \end{tabular}
\end{center}
\caption{\label{results} Zero-shot performance of models trained on CT-RATE dataset at the resolution of 512x512x256.}
\end{table*}

